A parallel integration method for solar system dynamics

We describe how long-term solar system orbit integration could be implemented on a parallel computer. The interesting feature of our algorithm is that each processor is assigned not to a planet or a pair of planets but to a time-interval. Thus, the 1st week, 2nd week,..., 1000th week of an orbit are computed concurrently. The problem of matching the input to the (n+1)-st processor with the output of the n-th processor can be solved efficiently by an iterative procedure. Our work is related to the so-called waveform relaxation methods in the computational mathematics literature, but is specialized to the Hamiltonian and nearly integrable nature of solar system orbits. Simulations on serial machines suggest that, for the reasonable accuracy requirement of 1" per century, our preliminary parallel algorithm running on a 1000-processor machine would be about 50 times faster than the fastest available serial algorithm, and we have suggestions for further improvements in speed.

==> figmac.tex <==
\input fonts

\input epsf

\expandafter
\ifx\csname Afour\endcsname\relax
\else
    \vsize=24.65truecm \hsize=15.94truecm
\fi

\expandafter
\ifx\csname draft\endcsname\relax
\else \input landscap
\fi

\def\psfigcall#1#2{\def\epsfsize##1##2{#2}\centerline{\epsfbox{#1}}}


\def\insfig[#1,#2,#3]#4.{\midinsert\parindent=0pt
           \vbox to #3 {\vss\psfigcall{#1}{#2}}
           \def\par{\endgraf\endinsert} \ninepoint
           \ignorespaces {\bf #4.}\quad \ignorespaces}


\def\blackout{\catcode`\\=12\catcode`\{=12\catcode`\}=12\catcode`\$=12
\catcode`\&=12\catcode`\#=12\catcode`\^=12\catcode`\_=12\catcode`\@=12
\catcode`\~=12\catcode`\%=12\catcode`\|=12}

{\obeylines \global\let
                       \relax
    \gdef\fig{\begingroup\obeylines\verbatim}
    \gdef\verbatim{\blackout\def
                   ##1
                   {\setbox0\hbox{##1}%
                    \ifdim\wd0<1pt \endgroup \else\immediate\write1{##1}\fi
                   }
   \string\figcap}}

\def\figcap[#1,#2,#3]#4.{\write1{\null\vfil
           \vbox to #3{\vss\string\psfigcall{#1}{#2}}}
    \write1{\bigskip\bigskip\centerline{\twelvebf #4}\vfil\string\eject}
    \bigskip\noindent{\bf\ignorespaces#4.}}


\let\bye\relax

\expandafter
\ifx\csname submission\endcsname\relax
      \let\adjustlinespacing\relax
      \def\bye{\vfill\eject\end}
      \let\fig=\insfig
\else \def\adjustlinespacing{\baselineskip=1.5\baselineskip}
      \adjustlinespacing
      \def\bye{\closeout1 \vfill\eject
               \leftline{\bf\uppercase{figure captions}}
               \openout1=pscalls \input captions \closeout1
               \vfill\supereject \input pscalls \end}
      \openout1=captions
\fi




==> fonts.tex <==
\font\caps=cmcsc10 at 10 truept
\font\fourteenrm=cmr10 scaled 1440
\font\twelvebf=cmbx10 scaled 1200
\font\tenbmit=cmmib10

%----------For ninepoint text (quotations)------------------
%-----------(no scriptscripts)------------------------------
\font\ninerm=cmr9
\font\ninei=cmmi9
\skewchar\ninei='177
\font\ninesy=cmsy9
\skewchar\ninesy='60
\font\nineit=cmti9
\font\ninesl=cmsl9
\font\ninebf=cmbx9
\font\ninett=cmtt9
%
\def\ninepoint{\textfont0=\ninerm \scriptfont0=\sevenrm 
              \def\rm{\fam0\ninerm}\relax
              \textfont1=\ninei \scriptfont1=\seveni 
              \def\mit{\fam1}\def\oldstyle{\fam1\ninei}\relax
              \textfont2=\ninesy \scriptfont2=\sevensy 
              \def\cal{\fam2}\relax
              \textfont3=\tenex \scriptfont3=\tenex 
              \def\it{\fam\itfam\nineit}\relax
              \textfont\itfam=\nineit
              \def\sl{\fam\slfam\ninesl}\relax
              \textfont\slfam=\ninesl
              \def\bf{\fam\bffam\ninebf}\relax
              \textfont\bffam=\ninebf \scriptfont\bffam=\sevenbf
              \def\tt{\fam\ttfam\ninett}\relax
              \textfont\ttfam=\ninett
              \setbox\strutbox=\hbox{\vrule
                   height8pt depth3pt width0pt}\baselineskip=11pt
              \adjustlinespacing
              \rm}



%----------For eightpoint text (footnotes)------------------
%-----------(no scriptscripts)------------------------------
\font\eightrm=cmr8
\font\eighti=cmmi8
\skewchar\eighti='177
\font\eightsy=cmsy8
\skewchar\eightsy='60
\font\eightit=cmti8
\font\eightsl=cmsl8
\font\eightbf=cmbx8
\font\eighttt=cmtt8
%
\def\eightpoint{\textfont0=\eightrm \scriptfont0=\fiverm 
                \def\rm{\fam0\eightrm}\relax
                \textfont1=\eighti \scriptfont1=\fivei 
                \def\mit{\fam1}\def\oldstyle{\fam1\eighti}\relax
                \textfont2=\eightsy \scriptfont2=\fivesy 
                \def\cal{\fam2}\relax
                \textfont3=\tenex \scriptfont3=\tenex 
                \def\it{\fam\itfam\eightit}\relax
                \textfont\itfam=\eightit
                \def\sl{\fam\slfam\eightsl}\relax
                \textfont\slfam=\eightsl
                \def\bf{\fam\bffam\eightbf}\relax
                \textfont\bffam=\eightbf \scriptfont\bffam=\fivebf
                \def\tt{\fam\ttfam\eighttt}\relax
                \textfont\ttfam=\eighttt
                \setbox\strutbox=\hbox{\vrule
                     height7pt depth2pt width0pt}\baselineskip=9pt
                \adjustlinespacing
                \rm}


==> macros.tex <==
\input figmac

\catcode`\@=11

%-----------------Footnotes---------------------------
\newcount\notenum

\def\vfootnote#1{\insert\footins\bgroup\eightpoint
     \interlinepenalty=\interfootnotelinepenalty
     \splittopskip=\ht\strutbox \splitmaxdepth=\dp\strutbox
     \floatingpenalty=20000
     \leftskip=0pt \rightskip=0pt \parskip=1pt \spaceskip=0pt \xspaceskip=0pt
     \smallskip\textindent{#1}\footstrut\futurelet\next\fo@t}

\def\note{\global\advance\notenum by 1
    \edef\n@tenum{$^{\the\notenum}$}\let\@sf=\empty
    \ifhmode\edef\@sf{\spacefactor=\the\spacefactor}\/\fi
    \n@tenum\@sf\vfootnote{\n@tenum}}


%------------Numbering equations-----------------------------

\newcount\eqnum
\def\nextenum{\global\advance\eqnum by 1
              \thenumber\rm}
\def\prevenum#1{{\advance\eqnum by -#1 \advance\eqnum by 1
                 \thenumber}\rm}
\def\name#1{\xdef#1{\thenumber}\ignorespaces}
\def\putnum{\eqno(\nextenum)}
\def\thenumber{\the\eqnum}

%--------------Abbreviations---------------------------------

\def\<#1>{{\left\langle#1\right\rangle}}

\def\witchbox#1#2#3{\hbox{$\mathchar"#1#2#3$}}
\def\leqsim{\mathrel{\rlap{\lower3pt\witchbox218}\raise2pt\witchbox13C}}
\def\geqsim{\mathrel{\rlap{\lower3pt\witchbox218}\raise2pt\witchbox13E}}

\let\twiddle=~ \def~{{}\ifmmode\widetilde\else\twiddle\fi}
\let\comma=\, \def\,{\ifmmode\comma\else\thinspace\fi}

\def\frac#1/#2{\mathchoice  {\hbox{$#1\over#2$}} {{#1\over#2}}
                {\scriptstyle{#1\over#2}}
                {#1\mskip-1.5mu/\mskip-1.5mu#2}}
\def\half{{\frac1/2}}

\def\pderiv(#1/#2){\mathchoice{\partial#1\over\partial#2}
    {\partial#1/\partial#2} {\partial#1/\partial#2} {\partial#1/\partial#2}}
\def\pderivp(#1/#2){\left(\pderiv(#1/#2)\right)}

\def\tderiv(#1/#2){\mathchoice{d#1\over d#2}{d#1/d#2}
                   {d#1/d#2}{d#1/d#2}}
\def\tderivp(#1/#2){\left(\tderiv(#1/#2)\right)}

\def\leftmatrix#1{\null\,\vcenter{\normalbaselines\m@th
    \ialign{$##$\hfil&&\quad$##$\hfil\crcr
      \mathstrut\crcr\noalign{\kern-\baselineskip}
      #1\crcr\mathstrut\crcr\noalign{\kern-\baselineskip}}}\,}

\def\rightmatrix#1{\null\,\vcenter{\normalbaselines\m@th
    \ialign{\hfil$##$&&\quad\hfil$##$\crcr
      \mathstrut\crcr\noalign{\kern-\baselineskip}
      #1\crcr\mathstrut\crcr\noalign{\kern-\baselineskip}}}\,}



%---------------Miscellaneous---------------------------------------

\headline={\ifnum\pageno=0\hfil
           \else\ifodd\pageno\hfil\tenit\rhead\quad\hbox{\tenbf\folio}%
                \else\hbox{\tenbf\folio}\quad\tenit\lhead\hfil\fi
           \fi}

\footline={\hfil}

\parskip \smallskipamount

\def\maybebreak#1{\vskip 0pt plus #1\vsize \penalty -1000
                  \vskip 0pt plus -#1\vsize}

\outer\def\section#1.#2\par{\maybebreak{.1}\bigskip\bigskip\bigskip
      \mark{#2} \centerline{\ninerm#1. \eightrm\uppercase{#2}}
      \medskip\noindent}
\outer\def\sectionlike#1\par{\maybebreak{.1}\bigskip\bigskip\bigskip
      \mark{#1} \centerline{\eightrm\uppercase{#1}}
      \medskip\noindent}

\def\comment{$\{$\bgroup\eightpoint\it\aftergroup\endcomment\let\next}
\def\endcomment{$\}$}

\def\ordsuffix#1{\ifcase#1\or st\or nd\or rd\or th\or th\or %6
    th\or th\or th\or th\or th\or th\or th\or th\or th\or %15
    th\or th\or th\or th\or th\or th\or st\or nd\or rd\or %24
    th\or th\or th\or th\or th\or th\or th\or st\fi}
\def\dayord#1{#1$^{\rm\ordsuffix{#1}}$}
\def\today{\expandafter\dayord{\number\day}
 \ifcase\month\or
 January\or February\or March\or April\or May\or June\or
 July\or August\or September\or October\or November\or December\fi
 \space \number\year}

\catcode`\@=12

\def\pseudocode{$$\vcenter\bgroup\dimen1=\parindent
        \advance\hsize by -2\dimen1
        \rightskip=\dimen1\parindent=0pt
        \def\begin{\par\advance\leftskip by \dimen1}
        \def\nigeb{\par\advance\leftskip by -\dimen1}
        \setbox1\hbox{$\langle\,$}
        \def\<{\hangindent\wd1\hangafter1$\langle\,$}
        \def\>{$\,\rangle$\par}}
\def\endcode{\egroup\eqno\vrule height0pt width.1pt depth0pt
                         \llap{(\nextenum)}$$}

%-----------------Local stuff-----------------------------------------------

\def\zmid#1#2{\left(\half(z_{#1}+z_{#2})\right)}
\def\zpmid#1#2{\left(\half(p_{#1}+p_{#2})\right)}
\def\Hzer{H^{\scriptscriptstyle(0)}}  \def\Hone{H^{\scriptscriptstyle(1)}}
\def\Herr{H_{\rm err}}

\font\syvec=cmbsy10
\def\bnabla{\hbox{\syvec\char114}}
\def\z{{\bf z}} \def\w{{\bf w}}
\def\I{{\bf I}} \def\J{{\bf J}} \def\Jinv{{\bf J}^{-1}}
\def\x{{\bf x}} \def\y{{\bf y}}

\def\WH{{\ninerm WH}91}  \def\ST{{\ninerm ST}94}  \def\WHT{{\ninerm WHT}94}

\expandafter\ifx\csname submission\endcsname\relax
                \def\figsize{.7\hsize}%
            \else\let\figsize\hsize
            \fi
% Makes figures bigger in the submission version.


